Latent Skill Planning for Exploration and Transfer

To quickly solve new tasks in complex environments, intelligent agents need to build up reusable knowledge. For example, a learned world model captures knowledge about the environment that applies to new tasks. Similarly, skills capture general behaviors that can apply to new tasks. In this paper, we investigate how these two approaches can be integrated into a single reinforcement learning agent. Specifically, we leverage the idea of partial amortization for fast adaptation at test time. For this, actions are produced by a policy that is learned over time while the skills it conditions on are chosen using online planning. We demonstrate the benefits of our design decisions across a suite of challenging locomotion tasks and demonstrate improved sample efficiency in single tasks as well as in transfer from one task to another, as compared to competitive baselines. Videos are available at: https://sites.google.com/view/latent-skill-planning/

==> agent.tex <==
% \begin{algorithm}[h!]
%     %\begin{algorithmic}[1] % The number tells where the line numbering should start
%     \State Initialize environment transitions data $\mathcal{D} \shortleftarrow \{ \}$
%     \For{Trial m=1 to M}
%         \State Train dynamics model $s_{1:T}=f_\phi(a_{1:T}, s_1)$, reward model $R_\zeta(s_{1:T})$ with $\mathcal{D}$
%                 %\State // \texttt{If goal-conditioned, sample a goal here}
%         \For {Environment Step l=1 to L}  // \texttt{Start of the episode}
%             \State Sample $G$ initial plans $\{{z_{1:\ceil{T/K}}}^{(0)}\}_{g=1}^G$ from prior $p(z|\theta^{(0)})$
%             \For{CEM Iteration i=1 to I}
%                 %Obtain N action sequences $\{\bar{a}\}$ with $g$ conditioned on $\{\widetilde{s}(\tau)\}$ acting under $f$
%                 \State Calculate model returns for plans $R_g^{(i)}=\sum_\tau r(s_\tau)$,  $\quad s_{\tau+1} = f(q_\phi(s_\tau, z_{\floor{\tau/p}}^{(i)}))$ 
%                 \State Sort $\{{z_{0:\ceil{H/p}}}^{(0)}\}_{g=1}^G$ based on total model returns
%                 \State Update $\theta^{(i)} = (\mu^{(i)}_{1:K},\Sigma^{(i)}_{1:K})$ to match the top action sequences and resample plans
%             \EndFor
%             \State Train $q_\phi(a|s,z)$ through SAC with $p(z|\theta^{(I)})$
%             \State Execute first action from the highest model return action sequence
%       \EndFor 
%   \EndFor 
%     %\end{algorithmic}
%     \caption{Hierarchical Planning Algorithm (The proposed approach)}
%     \label{alg:algorithm}
% \end{algorithm}

\begin{algorithm}[b]
%\small
\SetEndCharOfAlgoLine{}
\SetKwComment{Comment}{// }{}
%\begin{minipage}[t]{.62\textwidth}%
\BlankLine
Initialize dataset $\mathcal{D}$ with $S$ random seed episodes. \;
Initialize neural network parameters $\theta,\phi,\psi$ randomly. \;
Representation $\pr[p_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1},o_t)$ \;
Transition $\pr[q_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1})$ \;
Reward $\pr[q_\theta](r_t|s_t)$ \;
Action $\pr[q_\phi](a_t|s_t,z)$ \;
Value $\pr[v_\psi](s_t)$\;
Skill Distribution  $p(z|\zeta)$ \;
Backward skill prediction model $f_\chi(z|\{s\})$\;
Intrinsic reward $r^i(z,\{s\})=-||z-f_\chi(z|\{s\})||_2$ \;
\While{not converged}{
  \For{update step $c=1..C$}{
    \BlankLine\Comment{Dynamics learning}
    Draw $B$ data sequences $\{(a_t,o_t,r_t)\}_{t=k}^{k+L}\sim\mathcal{D}$. \;
    Compute model states $s_t\sim\pr[p_\theta](s_t|s_{t-1},a_{t-1},o_t)$. \;
    Update $\theta$ using representation learning. \;
    \BlankLine\Comment{Behavior learning}
    % Sample $K$ skill-commitments $p_k\sim\texttt{Cat}([P_{min},P_{max}])$  \;
    % \textbf{Assert} $\sum_{k=1}^{K-1}p_k\leq H$ and $\sum_{k=1}^{K}p_k\geq H$\;
     Sample $G$ initial skills $\{z^{(0)}\}_{g=1}^G$ from prior $p(z|\zeta^{(0)})$ \;
      \For{j in range(MaxCEMiter)}{ 
    \For{g in range(G)}{ 
     // \texttt{Imagine trajectories $\{(s_\tau,a_\tau)\}_{\tau=t}^{t+H}$ from each $s_t$. \;}
    \For{each $s_t$}{
    $\tau=t$\;
    
    \While{$\tau<H$}{
    
    %Sample skill $z_{\tau}\sim\pr[q_\zeta](\cdot|s_{\tau})$ \;
    
     Sample action $a_{\tau}\sim\pr[q_\phi](a_{\tau}|s_{\tau},z^{(j)})$\;
     Observe new state $s_{\tau+1}$ and compute new intrinsic reward $r_i$\;
   
    }
    }
    
    // \texttt{For high level planner}\;
    Predict rewards $R_g=\E{}{\pr[q_\theta](r_\tau|s_\tau)}$\;
    %  Sample $K$ skill-commitments $p_k\sim\texttt{Cat}([P_{min},P_{max}])$  \;
    % \textbf{Assert} $\sum_{k=1}^{K-1}p_k\leq H$ and $\sum_{k=1}^{K}p_k\geq H$\;
    %  Sample $G$ initial plans $\{{z_{1:K}}^{(0)}\}_{g=1}^G$ from prior $p(z|\zeta^{(0)})$ \;
    }
    
    \textbf{Sort} $\{R_g\}_{g=1}^G$ and use the top M sequences to update $\zeta^{(j)} = (\mu^{(j)},\Sigma^{(j)})$\;
        Sample $G$  skills $\{z^{(j)}\}_{g=1}^G$ from $p(z|\zeta^{(j)})$ \;
    }
    // \texttt{ Add Gaussian noise for diverse skills} \;
    $\mu^{(MaxCEMiter)} = \mu^{(MaxCEMiter)}+ \epsilon$ \;
     // \texttt{For low level policy}\;
    Compute rewards $R=\E{}{\pr[q_\theta](r_\tau|s_\tau)}$ with the optimized CEM distribution \;
    Compute the corresponding intrinsic rewards $r^i$\;
    Store the corresponding states into $K-$sized sequences $\{\{s\}_k \}_{k=1}^{\ceil{H/K}}$\;
    Use total rewards $R+r^i$, compute values $v_\psi(s_\tau)$ and compute value estimates $\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)$ \;
    
    Update $\phi\leftarrow\phi+\alpha\nabla_\phi\sum_{\tau=t}^{t+H}\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)$. // \texttt{For low level policy}\;
    
    Update $\shortpsi\leftarrow\shortpsi-\alpha\nabla_\psi\sum_{\tau=t}^{t+H}\frac{1}{2}\big\|v_\psi(s_\tau)\!\shortminus\!\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)\big\|^2$.// \texttt{For low level policy}\;
    
     Update $\chi\leftarrow\chi-\alpha\nabla_\chi\sum_{k=1}^{\ceil{H/K}}\frac{1}{2}\big\|z-f_\chi(\{s\}_k)\big\|^2$.// \texttt{For skill predictor}\;
  }
  \BlankLine\Comment{Environment interaction}
  $o_1\leftarrow\texttt{env.reset()}$ \;
  Sample skill $z$ from $p(z|\zeta^{(MaxCEMiter)})$ \;
  \For{time step $t=1..T$}{
        // \texttt{MPC in z space. Resample skill every K timesteps}\;
\If{$t\%K==0$}{ 
 Sample skill $z$ from $p(z|\zeta^{(MaxCEMiter)})$ \;
}
    Compute $s_t\sim\pr[p_\theta](s_t|s_{t-1},a_{t-1},o_t)$ from history. \;
    Compute $a_t\sim\pr[q_\phi](a_t|s_t,z)$ with the action model. \;
    Add exploration noise to action. \;
    $r_t,o_{t+1}\leftarrow\texttt{env.step(}a_t\texttt{)}.$ \;
  }
  Add experience to dataset $\mathcal{D}\leftarrow\mathcal{D}\cup\{(o_t,a_t,r_t)_{t=1}^T\}.$ \;
  \BlankLine
}
% \end{minipage}%
% \begin{minipage}[t]{.38\textwidth}%
% \vspace{1ex}%
% \textbf{Model components} \\
% \begin{tabular}[t]{@{} p{7em} @{} l @{}}%
% Representation & $\pr[p_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1},o_t)$ \\
% Transition & $\pr[q_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1})$ \\
% Reward & $\pr[q_\theta](r_t|s_t)$ \\
% Action & $\pr[q_\phi](a_t|s_t)$ \\
% Value & $\pr[v_\psi](s_t)$ \vspace{1ex} \\
% \end{tabular}
% \textbf{Hyper parameters} \\
% \begin{tabular}[t]{@{} p{14em} @{} c @{}}%
% Seed episodes & $S$ \\
% Collect interval & $C$ \\
% Batch size & $B$ \\
% Sequence length & $L$ \\
% Imagination horizon & $H$ \\
% Learning rate & $\alpha$ \\
% \end{tabular}
% \end{minipage}%
\caption{HI-PAPA Partial Amortized Version with Intrinsic Reward}
\label{alg:agent}
\end{algorithm}






% % \begin{itemize}
% %     \item Trivial way to add exploration bonus to CEM is to add a noise term $\epsilon$ while adapting the covariance.
% % \end{itemize}
% \begin{algorithm}[b]
% %\small
% \SetEndCharOfAlgoLine{}
% \SetKwComment{Comment}{// }{}
% %\begin{minipage}[t]{.62\textwidth}%
% \BlankLine
% Initialize dataset $\mathcal{D}$ with $S$ random seed episodes. \;
% Initialize neural network parameters $\theta,\phi,\psi$ randomly. \;
% Representation $\pr[p_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1},o_t)$ \;
% Transition $\pr[q_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1})$ \;
% Reward $\pr[q_\theta](r_t|s_t)$ \;
% Action $\pr[q_\phi](a_t|s_t,z_t)$ \;
% Value $\pr[v_\psi](s_t)$\;
% Skill Distribution  $p(z|\zeta)$ \;
% Intrinsic reward $r_i(s_t,z_t,a_t,s_{t+1})=-||s_t+z_t-s_{t+1}||_2$ (The choice of this is to be discussed)\;
% \While{not converged}{
%   \For{update step $c=1..C$}{
%     \BlankLine\Comment{Dynamics learning}
%     Draw $B$ data sequences $\{(a_t,o_t,r_t)\}_{t=k}^{k+L}\sim\mathcal{D}$. \;
%     Compute model states $s_t\sim\pr[p_\theta](s_t|s_{t-1},a_{t-1},o_t)$. \;
%     Update $\theta$ using representation learning. \;
%     \BlankLine\Comment{Behavior learning}
%     % Sample $K$ skill-commitments $p_k\sim\texttt{Cat}([P_{min},P_{max}])$  \;
%     % \textbf{Assert} $\sum_{k=1}^{K-1}p_k\leq H$ and $\sum_{k=1}^{K}p_k\geq H$\;
%      Sample $G$ initial plans $\{{z_{1:K}}^{(0)}\}_{g=1}^G$ from prior $p(z|\zeta^{(0)})$ \;
%       \For{j in range(MaxCEMiter)}{ 
%     \For{g in range(G)}{ 
%      // \texttt{Imagine trajectories $\{(s_\tau,a_\tau)\}_{\tau=t}^{t+H}$ from each $s_t$. \;}
%     \For{each $s_t$}{
%     $\tau=t$, $p=\ceil{H/K}$\;
    
%     \While{$\tau<H$}{
    
%     %Sample skill $z_{\tau}\sim\pr[q_\zeta](\cdot|s_{\tau})$ \;
%     \For{$\tau'=\tau....(\tau+p)$}{
%      Sample action $a_{\tau'}\sim\pr[q_\phi](a_{\tau'}|s_{\tau'},z_{\tau})$\;
%      Observe new state $s_{\tau+1}$ and compute new intrinsic reward $r_i$\;
%     }
%     $\tau=\tau+p$
%     }
%     }
    
%     // \texttt{For high level planner}\;
%     Predict rewards $R_g=\E{}{\pr[q_\theta](r_\tau|s_\tau)}$\;
%     %  Sample $K$ skill-commitments $p_k\sim\texttt{Cat}([P_{min},P_{max}])$  \;
%     % \textbf{Assert} $\sum_{k=1}^{K-1}p_k\leq H$ and $\sum_{k=1}^{K}p_k\geq H$\;
%     %  Sample $G$ initial plans $\{{z_{1:K}}^{(0)}\}_{g=1}^G$ from prior $p(z|\zeta^{(0)})$ \;
%     }
    
%     \textbf{Sort} $\{R_g\}_{g=1}^G$ and use the top M sequences to update $\zeta^{(j)} = (\mu^{(j)}_{1:K},\Sigma^{(j)}_{1:K})$\;
%     $\zeta^{(j)}= \zeta^{(j)} + \epsilon$ // \texttt{$\epsilon$ is a Gaussian noise for exploration}\;
%     Sample $G$  plans $\{{z_{1:K}}^{(0)}\}_{g=1}^G$ from $p(z|\zeta^{(j)})$ \;
%     }
%      // \texttt{For low level policy}\;
%     Compute rewards $R=\E{}{\pr[q_\theta](r_\tau|s_\tau)}$ with the optimized CEM distribution \;
%     Compute the corresponding intrinsic rewards $r_i$\;
%     Use total rewards $R+r_i$, compute values $v_\psi(s_\tau)$ and compute value estimates $\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)$ \;
    
%     Update $\phi\leftarrow\phi+\alpha\nabla_\phi\sum_{\tau=t}^{t+H}\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)$. // \texttt{For low level policy}\;
    
%     Update $\shortpsi\leftarrow\shortpsi-\alpha\nabla_\psi\sum_{\tau=t}^{t+H}\frac{1}{2}\big\|v_\psi(s_\tau)\!\shortminus\!\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)\big\|^2$.// \texttt{For low level policy}\;
%   }
%   \BlankLine\Comment{Environment interaction}
%   $o_1\leftarrow\texttt{env.reset()}$ \;
%   Sample $G$  plans $\{{z_{1:K}}^{(0)}\}_{g=1}^G$ from $p(z|\zeta^{(MaxCEMiter)})$ \;
%   \For{time step $t=1..T$}{
%     $p = \ceil{t/K}$ \;
%     Compute $s_t\sim\pr[p_\theta](s_t|s_{t-1},a_{t-1},o_t)$ from history. \;
%     Compute $a_t\sim\pr[q_\phi](a_t|s_t,z_p)$ with the action model. \;
%     Add exploration noise to action. \;
%     $r_t,o_{t+1}\leftarrow\texttt{env.step(}a_t\texttt{)}.$ \;
%   }
%   Add experience to dataset $\mathcal{D}\leftarrow\mathcal{D}\cup\{(o_t,a_t,r_t)_{t=1}^T\}.$ \;
%   \BlankLine
% }
% % \end{minipage}%
% % \begin{minipage}[t]{.38\textwidth}%
% % \vspace{1ex}%
% % \textbf{Model components} \\
% % \begin{tabular}[t]{@{} p{7em} @{} l @{}}%
% % Representation & $\pr[p_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1},o_t)$ \\
% % Transition & $\pr[q_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1})$ \\
% % Reward & $\pr[q_\theta](r_t|s_t)$ \\
% % Action & $\pr[q_\phi](a_t|s_t)$ \\
% % Value & $\pr[v_\psi](s_t)$ \vspace{1ex} \\
% % \end{tabular}
% % \textbf{Hyper parameters} \\
% % \begin{tabular}[t]{@{} p{14em} @{} c @{}}%
% % Seed episodes & $S$ \\
% % Collect interval & $C$ \\
% % Batch size & $B$ \\
% % Sequence length & $L$ \\
% % Imagination horizon & $H$ \\
% % Learning rate & $\alpha$ \\
% % \end{tabular}
% % \end{minipage}%
% \caption{HI-PAPA Partial Amortized Version with Intrinsic Reward}
% \label{alg:agent}
% \end{algorithm}




% \begin{algorithm}[b]
% %\small
% \SetEndCharOfAlgoLine{}
% \SetKwComment{Comment}{// }{}
% %\begin{minipage}[t]{.62\textwidth}%
% \BlankLine
% Initialize dataset $\mathcal{D}$ with $S$ random seed episodes. \;
% Initialize neural network parameters $\theta,\phi,\psi$ randomly. \;
% Representation $\pr[p_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1},o_t)$ \;
% Transition $\pr[q_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1})$ \;
% Reward $\pr[q_\theta](r_t|s_t)$ \;
% Action $\pr[q_\phi](a_t|s_t,z_t)$ \;
% Value $\pr[v_\psi](s_t)$\;
% Skill Value $\pr[v_\chi](s_t)$\;
% Skill policy  $\pr[q_\zeta](z_t|s_t)$ \;
% Intrinsic reward $r_i(s_t,z_t,a_t,s_{t+1})=-||s_t+z_t-s_{t+1}||_2$ (The choice of this is to be discussed)\;
% \While{not converged}{
%   \For{update step $c=1..C$}{
%     \BlankLine\Comment{Dynamics learning}
%     Draw $B$ data sequences $\{(a_t,o_t,r_t)\}_{t=k}^{k+L}\sim\mathcal{D}$. \;
%     Compute model states $s_t\sim\pr[p_\theta](s_t|s_{t-1},a_{t-1},o_t)$. \;
%     Update $\theta$ using representation learning. \;
%     \BlankLine\Comment{Behavior learning}
%      //\texttt{Imagine trajectories $\{(s_\tau,a_\tau)\}_{\tau=t}^{t+H}$ from each $s_t$. \;}
%     \For{each $s_t$}{
%     $\tau=t$\;
%     \While{$\tau<H$}{
%     Sample skill-commitment $p\sim\texttt{Cat}([P_{min},P_{max}])$ \;
%     Sample skill $z_{\tau}\sim\pr[q_\zeta](\cdot|s_{\tau})$ \;
%     \For{$\tau'=\tau....(\tau+p)$}{
%      Sample action $a_{\tau'}\sim\pr[q_\phi](a_{\tau'}|s_{\tau'},z_{\tau})$\;
%      Observe new state $s_{\tau+1}$ and compute new intrinsic reward $r_i$\;
%     }
%     $\tau=\tau+p$
%     }
%     }
%     // \texttt{For high level policy}\;
%     Predict rewards $\E{}{\pr[q_\theta](r_\tau|s_\tau)}$ and values $v_\chi(s_\tau).$ Compute value estimates $\mathrm{V}_{\mathrm{\lambda}}(s_\tau)$  \;
%      // \texttt{For low level policy}\;
%     Use total rewards $r_i+R$, compute values $v_\psi(s_\tau)$ and compute value estimates $\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)$ \;
%     Update $\zeta\leftarrow\zeta+\alpha\nabla_\zeta\sum_{\tau=t}^{t+H}\mathrm{V}_{\mathrm{\lambda}}(s_\tau)$.  // \texttt{For high level policy}\;
%     Update $\phi\leftarrow\phi+\alpha\nabla_\phi\sum_{\tau=t}^{t+H}\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)$. // \texttt{For low level policy}\;
%     Update $\chi\leftarrow\chi-\alpha\nabla_\chi\sum_{\tau=t}^{t+H}\frac{1}{2}\big\|v_\chi(s_\tau)\!\shortminus\!\mathrm{V}_{\mathrm{\lambda}}(s_\tau)\big\|^2$.// \texttt{For high level policy}\;
%      Update $\shortpsi\leftarrow\shortpsi-\alpha\nabla_\psi\sum_{\tau=t}^{t+H}\frac{1}{2}\big\|v_\psi(s_\tau)\!\shortminus\!\mathrm{V}^i_{\mathrm{\lambda}}(s_\tau)\big\|^2$.// \texttt{For low level policy}\;
%   }
%   \BlankLine\Comment{Environment interaction}
%   $o_1\leftarrow\texttt{env.reset()}$ \;
%   \For{time step $t=1..T$}{
%     Compute $s_t\sim\pr[p_\theta](s_t|s_{t-1},a_{t-1},o_t)$ from history. \;
%     Compute $a_t\sim\pr[q_\phi](a_t|s_t)$ with the action model. \;
%     Add exploration noise to action. \;
%     $r_t,o_{t+1}\leftarrow\texttt{env.step(}a_t\texttt{)}.$ \;
%   }
%   Add experience to dataset $\mathcal{D}\leftarrow\mathcal{D}\cup\{(o_t,a_t,r_t)_{t=1}^T\}.$ \;
%   \BlankLine
% }
% % \end{minipage}%
% % \begin{minipage}[t]{.38\textwidth}%
% % \vspace{1ex}%
% % \textbf{Model components} \\
% % \begin{tabular}[t]{@{} p{7em} @{} l @{}}%
% % Representation & $\pr[p_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1},o_t)$ \\
% % Transition & $\pr[q_\theta](s_t|s_{t\text{-}1},a_{t\text{-}1})$ \\
% % Reward & $\pr[q_\theta](r_t|s_t)$ \\
% % Action & $\pr[q_\phi](a_t|s_t)$ \\
% % Value & $\pr[v_\psi](s_t)$ \vspace{1ex} \\
% % \end{tabular}
% % \textbf{Hyper parameters} \\
% % \begin{tabular}[t]{@{} p{14em} @{} c @{}}%
% % Seed episodes & $S$ \\
% % Collect interval & $C$ \\
% % Batch size & $B$ \\
% % Sequence length & $L$ \\
% % Imagination horizon & $H$ \\
% % Learning rate & $\alpha$ \\
% % \end{tabular}
% % \end{minipage}%
% \caption{HI-PAPA}
% \label{alg:agent}
% \end{algorithm}

==> behavior.tex <==
% \section{Learning Temporally-Abstracted Behaviors by Latent Imagination}
% \label{sec:behavior}
% \vspace{-1ex}
\section*{}
\label{sec:behavior}

%\input{figures/schema/figure}
\input{agent}
%\input{figures/horizon/figure}

% Dreamer learns long-horizon behaviors in the compact latent space of a learned world model by efficiently leveraging the neural network latent dynamics. For this, we propagate stochastic gradients of multi-step returns through neural network predictions of actions, states, rewards, and values using reparameterization. This section describes the main contribution of our paper.

% \paragraph{Imagination environment}

% The latent dynamics define a Markov decision process \citep[MDP;][]{sutton1991dyna} that is fully observed because the compact model states $s_t$ are Markovian. We denote imagined quantities with $\tau$ as the time index. Imagined trajectories start at the true model states $s_t$ of observation sequences drawn from the agent's past experience. They follow predictions of the transition model $s_\tau\sim\q(s_\tau|s_{\tau-1},a_{\tau-1})$, reward model $r_\tau\sim\q(r_\tau|s_\tau)$, and a policy $a_\tau\sim\q(a_\tau|s_\tau)$. The objective is to maximize expected imagined rewards $\smash{\E{q}{\sum_{\tau=t}^\infty \gamma^{\tau-t} r_\tau}}$ with respect to the policy.

% \paragraph{Action and value models}

% Consider imagined trajectories with a finite horizon $H$. Dreamer uses an actor critic approach to learn behaviors that consider rewards beyond the horizon. We learn an action model and a value model in the latent space of the world model for this. The action model implements the policy and aims to predict actions that solve the imagination environment. The value model estimates the expected imagined rewards that the action model achieves from each state $s_\tau$,
% \begin{equation}
% \begin{aligned}
% \makebox[12em][l]{Action model:} && &a_\tau \sim\ \pr[q_\phi](a_\tau|s_\tau) \\
% \makebox[12em][l]{Value model:} && &v_\psi(s_\tau) \approx \E{q(\cdot|s_\tau)}{\textstyle\sum_{\tau=t}^{t+H}\gamma^{\tau-t}r_\tau}.
% \label{eq:action_value_model}
% \end{aligned}
% \end{equation}%
% The action and value models are trained cooperatively as typical in policy iteration: the action model aims to maximize an estimate of the value, while the value model aims to match an estimate of the value that changes as the action model changes.

% We use dense neural networks for the action and value models with parameters $\phi$ and $\psi$, respectively. The action model outputs a tanh-transformed Gaussian \citep{haarnoja2018sac} with sufficient statistics predicted by the neural network. This allows for reparameterized sampling \citep{kingma2013vae,rezende2014vae} that views sampled actions as deterministically dependent on the neural network output, allowing us to backpropagate analytic gradients through the sampling operation,
% \begin{equation}
% a_\tau=\operatorname{tanh}\!\big(\mu_\phi(s_\tau)+\sigma_\phi(s_\tau)\,\epsilon\big),
% \quad\epsilon\sim\Normal(0,\I).
% \end{equation}%

% \paragraph{Value estimation}

% To learn the action and value models, we need to estimate the state values of imagined trajectories $\{s_\tau,a_\tau,r_\tau\}_{\tau=t}^{t+H}$. These trajectories branch off of the model states $s_t$ of sequence batches drawn from the agent's dataset of experience and predict forward for the imagination horizon $H$ using actions sampled from the action model. State values can be estimated in multiple ways that trade off bias and variance \citep{sutton2018rl},
% \begin{alignat}{3}
% &\mathrm{V}_{\mathrm{R}}(s_\tau)&&\defined\E[\bigg]{q_\theta,q_\phi}{
%     \sum_{n=\tau}^{t+H} r_n}, \\
% &\mathrm{V}_{\mathrm{N}}^k(s_\tau)&&\defined\E[\bigg]{q_\theta,q_\phi}{
%     \sum_{n=\tau}^{h-1} \gamma^{n-\tau}r_n
%     +\gamma^{h-\tau} v_\psi(s_h)} \quad\text{with}\quad h=\min(\tau+k,t+H), \\
% &\mathrm{V}_{\mathrm{\lambda}}(s_\tau)&&\defined
%     (1-\lambda) \sum_{n=1}^{H-1} \lambda^{n-1} \mathrm{V}_{\mathrm{N}}^n(s_\tau) + \lambda^{H-1}\mathrm{V}_{\mathrm{N}}^H(s_\tau),
% \label{eq:lambda_value}
% \end{alignat}%
% where the expectations are estimated under the imagined trajectories. $\mathrm{V}_{\mathrm{R}}$ simply sums the rewards from $\tau$ until the horizon and ignores rewards beyond it. This allows learning the action model without a value model, an ablation we compare to in our experiments. $\mathrm{V}_{\mathrm{N}}^k$ estimates rewards beyond $k$ steps with the learned value model. Dreamer uses $\mathrm{V}_{\mathrm{\lambda}}$, an exponentially-weighted average of the estimates for different $k$ to balance bias and variance. \Cref{fig:horizon} shows that learning a value model in imagination enables Dreamer to solve long-horizon tasks while being robust to the imagination horizon. The experimental details and results on all tasks are described in \cref{sec:experiments}.

% \pagebreak

% \paragraph{Learning objective}

% To update the action and value models, we first compute the value estimates $\mathrm{V}_{\mathrm{\lambda}}(s_\tau)$ for all states $s_\tau$ along the imagined trajectories. The objective for the action model $\pr[q_\phi](a_\tau|s_\tau)$ is to predict actions that result in state trajectories with high value estimates. The objective for the value model $v_\psi(s_\tau)$, in turn, is to regress the value estimates,

% \noindent\begin{minipage}{.4\textwidth}\vspace*{-2ex}\hfil\begin{equation}
% \max_\phi\E[\bigg]{q_\theta,q_\phi}{\sum_{\tau=t}^{t+H} \mathrm{V}_{\mathrm{\lambda}}(s_\tau)}, \label{eq:action_objective} \\
% \end{equation}\end{minipage}%
% \noindent\begin{minipage}{.6\textwidth}\begin{equation}
% \min_\psi\E[\bigg]{q_\theta,q_\phi}{\sum_{\tau=t}^{t+H} \frac{1}{2}\Big\|v_\psi(s_\tau)-\mathrm{V}_{\mathrm{\lambda}}(s_\tau))\Big\|^2}. \label{eq:value_objective}
% \end{equation}\end{minipage}

% The value model is updated to regress the targets, around which we stop the gradient as typical \citep{sutton2018rl}. The action model uses analytic gradients through the learned dynamics to maximize the value estimates. To understand this, we note that the value estimates depend on the reward and value predictions, which depend on the imagined states, which in turn depend on the imagined actions. Since all steps are implemented as neural networks, we analytically compute $\smash{\nabla_\phi\E{q_\theta,q_\phi}{\sum_{\tau=t}^{t+H}\mathrm{V}_{\mathrm{\lambda}}(s_\tau)}}$ by stochastic backpropagation \citep{kingma2013vae,rezende2014vae}.
% We use reparameterization for continuous actions and latent states and straight-through gradients \citep{bengio2013straight} for discrete actions. The world model is fixed while learning behaviors.

% In tasks with early termination, the world model also predicts the discount factor from each latent state to weigh the time steps in \cref{eq:action_objective,eq:value_objective} by the cumulative product of the predicted discount factors, so terms are weighted down based on how likely the imagined trajectory would have ended.

% \paragraph{Comparison to actor critic methods}

% Agents using Reinforce gradients \citep{williams1992reinforce}, such as A3C and PPO \citep{mnih2016a3c,schulman2017ppo}, employ value baselines to reduce gradient variance, while Dreamer backpropagates through the value model. This is similar to deterministic or reparameterized actor critics \citep{silver2014dpg}, such as DDPG and SAC \citep{lillicrap2015ddpg,haarnoja2018sac}. However, these do not leverage gradients through transitions and only maximize immediate Q-values. MVE and STEVE \citep{feinberg2018mve,buckman2018steve} extend them to multi-step Q-learning with learned dynamics to provide more accurate Q-value targets. We predict state values, which is sufficient for policy optimization since we backpropagate through the dynamics. Refer to \cref{sec:related} for a more detailed comparison to related work.

==> macros.tex <==
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Acal}{\mathcal{A}}

\newcommand{\vr}{\mathbf{r}}
\newcommand{\eps}{\epsilon}
\newcommand{\book}{book\xspace}
\newcommand{\cX}{\ensuremath{\mathcal{X}}}
\newcommand{\cA}{\ensuremath{\mathcal{A}}}
\newcommand{\cP}{\ensuremath{\mathcal{P}}}
\newcommand{\cR}{\ensuremath{\mathcal{R}}}
\newcommand{\Xset}{\ensuremath{\mathcal{X}}}
\newcommand{\Aset}{\ensuremath{\mathcal{A}}}
\newcommand{\dist}{\ensuremath{D}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
%\DeclareMathOperator*{\EE}{{\mathbb{E}}}
%\DeclareMathOperator{\E}{{\mathbb{E}}}
%\DeclareMathOperator{\Eh}{\widehat{\mathbb{E}}}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\E}{\ensuremath{\mathbb{E}}}
\newcommand{\Eh}{\widehat{\mathbb{E}}}

\renewcommand{\P}{\mathbb{P}}
\newcommand{\F}{\ensuremath{\mathcal{F}}}
\renewcommand{\H}{\ensuremath{\mathcal{H}}}
%\newcommand{\E}{\ensuremath{\mathbb{E}}}
\DeclareMathOperator{\Var}{Var}
%\newcommand{\Var}{\text{\textup{Var}}}
\DeclareMathOperator{\argmax}{argmax}
\DeclareMathOperator{\argmin}{{argmin}}
\newcommand{\order}{\ensuremath{\mathcal{O}}}
\newcommand{\otil}{\ensuremath{\widetilde{\order}}}
\newcommand{\term}{\ensuremath{\mathcal{T}}}
\DeclareMathOperator{\BiasBdOp}{Bias}
\newcommand{\BiasBd}{\widehat{\BiasBdOp}}

\newcommand{\matM}{\mathbf{M}}
\newcommand{\vf}{\mathbf{f}}
\newcommand{\tvr}{\mathbf{\tilde{r}}}
\newcommand{\tr}{\tilde{r}}

\newcommand{\regret}{\ensuremath{\mathrm{Regret}}}
\newcommand{\reg}{\ensuremath{\mathrm{Reg}}}
\newcommand{\regh}{\ensuremath{\mathrm{\widehat{Reg}}}}
\newcommand{\vb}{\ensuremath{\mathbf{b}}}
\newcommand{\minprob}{\ensuremath{\gamma}}

\newcommand{\greedy}{\textsc{Greedy}\xspace}
\newcommand{\hedge}{\textsc{Hedge}\xspace}
\newcommand{\hedgep}{\ensuremath{\mathbf{p}}}
\newcommand{\hedgew}{\ensuremath{\mathbf{w}}}
\newcommand{\hedgeu}{\ensuremath{\mathbf{u}}}
%\newcommand{\kl}[2]{\ensuremath{\textrm{D}_{\textrm{KL}}\left( {#1}~||~{#2} \right)}}

\newcommand{\pihat}{\ensuremath{\widehat{\pi}}}
\newcommand{\w}{w}
\newcommand{\wmax}{\w_{\max}}
\newcommand{\hw}{\hat{w}}%\widehat{w}}
\newcommand{\hwmax}{\hw_{\max}}
\newcommand{\hr}{\hat{r}}%\widehat{r}}
\newcommand{\sr}{r^*}
\newcommand{\rmax}{R_{\max}}
\newcommand{\hV}{\hat{V}}%\widehat{V}}
\newcommand{\Xbar}{\ensuremath{\overline{X}}}
\newcommand{\event}{\ensuremath{\mathcal{E}}}
\newcommand{\piopt}{\ensuremath{\pi^\star}}
\newcommand{\ind}{\ensuremath{\mathds{1}}}
\newcommand{\alg}{\ensuremath{\operatorname{\mathtt{A}}}}

\newcommand{\Rexp}{\ensuremath{v}}%{\ensuremath{R}}%{\ensuremath{R^\star}}
\newcommand{\Rest}{\ensuremath{\widehat{v}}}%{\ensuremath{\widehat{R}}}
\newcommand{\Rpred}{\ensuremath{\widetilde{v}}}%{\ensuremath{\widetilde{R}}}
\newcommand{\ips}{\ensuremath{\texttt{\upshape IPS}}\xspace}
\newcommand{\dm}{\ensuremath{\texttt{\upshape DM}}\xspace}
\newcommand{\dr}{\ensuremath{\texttt{\upshape DR}}\xspace}
\newcommand{\switch}{\ensuremath{\texttt{\upshape SWITCH}}\xspace}
\newcommand{\Vhat}{\ensuremath{\widehat{V}}}
\newcommand{\mse}{\textup{\mdseries MSE}}

\newcommand{\AMO}{\ensuremath{\mathcal{AMO}\xspace}}
\newcommand{\pe}{\textsc{PolicyElimination}\xspace}


\newcommand{\pigood}{\ensuremath{\pi_{\textrm{good}}}}
\newcommand{\pibad}{\ensuremath{\pi_{\textrm{bad}}}}

\newcommand{\op}{\ensuremath{\mathsf{OP}}\xspace}
\newcommand\iltcb{\ensuremath{\mathsf{I LOVE TO CON BANDITS}}\xspace}

\newcommand{\Sset}{\ensuremath{\mathcal{S}}}
\newcommand{\Trans}{\ensuremath{P}}
\newcommand{\Rdist}{\ensuremath{r}}
\newcommand{\init}{\ensuremath{\nu}}
\newcommand{\Vstar}{\ensuremath{V^\star}}
\newcommand{\Qstar}{\ensuremath{Q^\star}}

\newcommand{\rmaxalg}{\textsc{R-Max}\xspace}
\newcommand{\rmaxe}{\textsc{R-Max-E}\xspace}
\newcommand{\rmaxg}{\textsc{R-Max-$\gamma$}\xspace}
\newcommand{\inith}{\ensuremath{\widehat{\init}}}
\newcommand{\Transh}{\ensuremath{\widehat{\Trans}}}
\newcommand{\Rdisth}{\ensuremath{\widehat{\Rdist}}}
\newcommand{\Mhat}{\ensuremath{\widehat{M}}}

\newcommand{\rhat}{\ensuremath{\widehat{r}}}

%% Theorems
% \theoremstyle{theorem}
% \newtheorem{theorem}{Theorem}[section]
% \newtheorem{lemma}{Lemma}[section]
% \newtheorem{corollary}{Corollary}[section]
% \newtheorem{claim}{Claim}[section]
% \newtheorem{assumption}{Assumption}[section]
% \theoremstyle{definition}
% \newtheorem{definition}{Definition}[section]
% \newtheorem{example}{Example}[section]
% \newtheorem{remark}{Remark}[section]
% \newtheorem*{lemma*}{Lemma}
% %\newtheorem*{remark}{Remark}
% \newtheorem{proposition}{Proposition}[section]
% \newtheorem{fact}{Fact}[section]
\renewenvironment{proof}{{\bf Proof:}}{\hfill\rule{2mm}{2mm}}
\newcommand{\Assume}[1]{Assumption~\ref{assume:#1}}
\newcommand{\Cor}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Fig}[1]{Figure~\ref{fig:#1}}
\newcommand{\Eq}[1]{Equation~\ref{eq:#1}}
\newcommand{\Sec}[1]{Section~\ref{sec:#1}}
\newcommand{\Thm}[1]{Theorem~\ref{thm:#1}}

% Parentheses
\newcommand{\card}[1]{\lvert#1\rvert}
\newcommand{\set}[1]{\{#1\}}
\newcommand{\Set}[1]{\left\{#1\right\}}
\newcommand{\bigSet}[1]{\bigl\{#1\bigr\}}
\newcommand{\BigSet}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\braces}[1]{\{#1\}}
\newcommand{\Braces}[1]{\left\{#1\right\}}
\newcommand{\bigBraces}[1]{\bigl\{#1\bigr\}}
\newcommand{\BigBraces}[1]{\Bigl\{#1\Bigr\}}
\newcommand{\bracks}[1]{[#1]}
\newcommand{\bigBracks}[1]{\bigl[#1\bigr]}
\newcommand{\BigBracks}[1]{\Bigl[#1\Bigr]}
\newcommand{\biggBracks}[1]{\biggl[#1\biggr]}
\newcommand{\BiggBracks}[1]{\Biggl[#1\Biggr]}
\newcommand{\Bracks}[1]{\left[#1\right]}
\newcommand{\parens}[1]{(#1)}
\newcommand{\Parens}[1]{\left(#1\right)}
\newcommand{\bigParens}[1]{\bigl(#1\bigr)}
\newcommand{\BigParens}[1]{\Bigl(#1\Bigr)}
\newcommand{\biggParens}[1]{\biggl(#1\biggr)}
\newcommand{\BiggParens}[1]{\Biggl(#1\Biggr)}
%\newcommand{\given}{\mathbin{\vert}}
\newcommand{\given}{|}
\newcommand{\bigGiven}{\mathbin{\bigm\vert}}
\newcommand{\BigGiven}{\mathbin{\Bigm\vert}}
\newcommand{\biggGiven}{\mathbin{\biggm\vert}}
\newcommand{\Norm}[1]{\left\lVert#1\right\rVert}
\newcommand{\bigNorm}[1]{\bigl\lVert#1\bigr\rVert}
\newcommand{\BigNorm}[1]{\Bigl\lVert#1\Bigr\rVert}
\newcommand{\norm}[1]{\lVert#1\rVert}
\newcommand{\abs}[1]{\lvert#1\rvert}
\newcommand{\Abs}[1]{\left\lvert#1\right\rvert}
\newcommand{\bigAbs}[1]{\bigl\lvert#1\bigr\rvert}
\newcommand{\BigAbs}[1]{\Bigl\lvert#1\Bigr\rvert}
\newcommand{\biggAbs}[1]{\biggl\lvert#1\biggr\rvert}
\newcommand{\angles}[1]{\langle#1\rangle}
\newcommand{\floors}[1]{\lfloor#1\rfloor}
\newcommand{\Floors}[1]{\left\lfloor#1\right\rfloor}
\newcommand{\ceils}[1]{\lceil#1\rceil}
\newcommand{\Eu}[1]{\underset{#1}{\E}}

\newcommand{\Vcal}{\ensuremath{\mathcal{V}}}
\newcommand{\Vcalh}{\ensuremath{\widehat{\mathcal{V}}}}
\newcommand{\Qtil}{\ensuremath{\tilde{Q}}}
\newcommand{\zhat}{\ensuremath{\hat{z}}}
\newcommand{\Vghat}{\ensuremath{{\Vhat}^\gamma}}
\newcommand{\err}{\ensuremath{\text{err}}}
\newcommand{\Hcal}{\ensuremath{\mathcal{H}}}
\newcommand{\Bell}{\ensuremath{\mathcal{T}}}
\newcommand{\Phat}{\ensuremath{\widehat P}}
\newcommand{\Bellh}{\ensuremath{\widehat \Bell}}
\newcommand{\calF}{\ensuremath{\mathcal{F}}}
\newcommand{\loss}{\ensuremath{\mathcal{L}}}
\newcommand{\lossh}{\ensuremath{\widehat{\loss}}}
\newcommand{\Qh}{\ensuremath{\widehat{Q}}}
\newcommand{\pitil}{\ensuremath{\widetilde{\pi}}}
\newcommand{\bp}{\ensuremath{\theta}}
\newcommand{\cntidx}{\ensuremath{\alpha}}
\newcommand{\bcnt}{\ensuremath{\bm{\cntidx}}}
\newcommand{\idx}{\ensuremath{\beta}}
\newcommand{\bidx}{\ensuremath{\bm{\idx}}}
\newcommand{\hist}{\ensuremath{\text{hist}}}
\newcommand{\mbound}{\ensuremath{\alpha}}
\newcommand{\pmax}{\ensuremath{\bar{p}}}
\newcommand{\pmin}{\ensuremath{\underline{p}}}
\renewcommand{\S}{\ensuremath{\mathbb{S}}}
\newcommand{\kl}{\ensuremath{\mathrm{KL}}}

\DeclareMathOperator{\chd}{child}

\newcommand{\epsopt}{\ensuremath{\eps_{\text{opt}}}}
\newcommand{\epsapp}{\ensuremath{\eps_{\text{approx}}}}
\newcommand{\lbpe}{\ensuremath{L_{\textrm{BPE}}}}
\newcommand{\tepsapp}{\ensuremath{\widetilde\eps_{\textrm{approx}}}}
\newcommand{\Ah}{\ensuremath{\widehat A}}
\newcommand{\wh}{\ensuremath{\widehat w}}
\newcommand{\epsh}{\ensuremath{\widehat{\eps}}}
\newcommand{\diag}{\textrm{diag}}
\newcommand{\ones}{\mathbf{1}}
\newcommand{\iden}{\textrm{I}}
\newcommand{\onesm}{\mathbf{J}}
\newcommand{\Wcal}{\ensuremath{\mathcal{W}}} 

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> mathnotes.tex <==

\begin{document}

$$ \mathcal{MI}(z,\{s\}|s_0) = \mathcal{H}(z|s_0) - \mathcal{H}(z|\{s\},s_0) = \mathcal{H}(\{s\}|s_0) - \mathcal{H}(\{s\},s_0|z) $$
Choice between modelling skill dynamics $q({s} | s_0, z)$ or skill predictor $q(z|s_0, {s})$.
With skill predictor:
$$ \mathcal{MI}(z,\{s\}|s_0) = \int p(z,\{s\},s_0)\log\frac{p(z|\{s\},s_0)}{p(z|s_0)}$$
$$ = \int p(z,\{s\},s_0)\log\frac{q(z|\{s\},s_0)}{p(z|s_0)}\frac{p(z|\{s\},s_0)}{q(z|\{s\},s_0)}$$
$$ \geq \int p(z,\{s\},s_0)\log\frac{q(z|\{s\},s_0)}{p(z|s_0)}$$
$$ = \int p(z,\{s\},s_0) \log q(z|\{s\},s_0) - \int p(z|s_0) \log p(z|s_0)$$
$$ = \mathbb{E}_{p(z,\{s\},s_0)}[\log q(z|\{s\},s_0)] + \mathcal{H}[p(z|s_0)]$$
$$p(z,\{s\},s_0) = p(z|s_0)p_\pi(\{s\}|z,s_0)p(s_0)$$

With skill dynamics $$\log p(\{s\}|z,s_0)=\log \prod_t p(s_{t+1}|s_t,a) \pi(a|s_t,z)$$
Marginal $$\log p(\{s\}|s_0)=\log \mathbb{E}_{z_i|s_0}\left[\prod_t p(s_{t+1}|s_t,a) \pi(a|s_t,z_i)\right]$$
$$ \mathcal{MI}(z,\{s\}|s_0) = \int p(z,\{s\},s_0)\log\frac{p(\{s\}|z,s_0)}{p(\{s\}|s_0)}$$
$$p(z,\{s\},s_0) = p(z|s_0)p_\pi(\{s\}|z,s_0)$$

$$ = \int p(z,\{s\},s_0)\log\frac{q(z|\{s\},s_0)}{p(z|s_0)}\frac{p(z|\{s\},s_0)}{q(z|\{s\},s_0)}$$
$$ \geq \int p(z,\{s\},s_0)\log\frac{q(z|\{s\},s_0)}{p(z|s_0)}$$

Do we amortize skill loss into value function?

\end{document}

==> notes/skill_pred_input_noise.tex <==

Although mutual information is a popular objective for skill discovery, it is important to 
When the underlying dynamics of the system are deterministic, a powerful world model may be able to model this accurately. In such a case the uncertainty in the distribution over future states given actions will approach 0.
This becomes an issue for the mutual information objective, when the agent is able to communicate the skill identity through a smaller subspace of the state space.
For example, image that in a quadruped walking task the height of a specific end effector at a certain future frame can be very confidently predicted by the dynamics model.
Whether to lift the end effector up 9cm or 10cm may be largely negligible in terms of the dynamics of the motion, but
the policy can choose to map the skill variable to the heights of a specific end effector at a certain future frame.

